Control Barrier Functions Solved with Hierarchical Quadratic Programming for Safe Physical Human-Robot Interaction

Physical human-robot interaction offers the potential to leverage human intelligence and robot physical capabilities to enable a range of exciting applications, e.g., collaborative robots for rehabilitation. Safety is critical for the successful deployment of this kind of robotic system. In recent years, Control Barrier Function (CBF) has emerged as an effective approach to enforce safety guarantees, which has been widely applied in various applications, from adaptive cruise control to navigation of legged robots. CBFs can be solved in a Quadratic Programming (QP) problem, which can include many CBF-formulated tasks. To manage a large number of safety tasks, a hierarchical CBF has been used to allow hierarchical relaxation of safety tasks to ensure the feasibility of a solution in the presence of conflicting tasks. In this work, we propose to use a CBF-based Hierarchical Quadratic Programming (HQP) framework in physical human-robot interaction to allow us to design both performance tasks (e.g., preserve the desired behavior at the human-robot interaction point) and safety tasks at any level of a hierarchy to balance the safety and the performance in a more flexible way. Extensive experiments were carried out on a real redundant robot to validate the effectiveness, flexibility, and generality of this approach.

==> mymacros.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Shorthands for greek letters %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% capital greek letters
\newcommand{\Ga}{\Gamma}
\newcommand{\De}{\Delta}
\newcommand{\Th}{\Tetha}
\newcommand{\La}{\Lambda}
\newcommand{\Si}{\Sigma}
\newcommand{\Ups}{\Upsilon}
\newcommand{\Om}{\Omega}

% lowercase greek letters
\newcommand{\al}{\alpha}
\newcommand{\be}{\beta}
\newcommand{\ga}{\gamma}
\newcommand{\de}{\delta}
\newcommand{\ep}{\varepsilon}
\renewcommand{\th}{\theta}  % In Times il comando \th produce una strana trombetta verticale.
\newcommand{\vth}{\vartheta}
\newcommand{\ka}{\kappa}
\newcommand{\la}{\lambda}
\newcommand{\si}{\sigma}
\newcommand{\vphi}{\varphi}
\newcommand{\om}{\omega}

% boldface greek letters
\newcommand{\bsi}{\boldsymbol{\si}}  %
\newcommand{\bga}{\boldsymbol{\ga}}  %
\newcommand{\bOm}{\boldsymbol{\Om}}  % vettore vel. angolare
\newcommand{\bom}{\boldsymbol{\om}}  % vettore quasi-coordinate
\newcommand{\bxi}{\boldsymbol{\xi}}  % twist in boldface
\newcommand{\bth}{\boldsymbol{\th}}  % vector of joint functions

% dotted greek letters
\newcommand{\dal}{\dot{\al}}
\newcommand{\dde}{\dot{\de}}
\newcommand{\dpsi}{\dot{\psi}}
\newcommand{\dth}{\dot{\th}}
\newcommand{\dphi}{\dot{\phi}}
\newcommand{\dvphi}{\dot{\vphi}}

\newcommand{\ddpsi}{\ddot{\psi}}
\newcommand{\ddth}{\ddot{\th}}
\newcommand{\ddphi}{\ddot{\phi}}

% hatted greek letters
\newcommand{\hxi}{\widehat{\xi}}
\newcommand{\home}{\widehat{\om}}

% hatted bold greek letters
\newcommand{\hbsi}{\hat{\bsi}}
\newcommand{\hbxi}{\hat{\bxi}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Shorthands for bold letters with boldsymbol    %%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% ********** WARNING  ************
% Use either this file boldsymbol.tex or file mathbf.tex, BUT NOT BOTH!!!

% Latin lowercase letters
\newcommand{\ba}{\boldsymbol{a}}
\newcommand{\bb}{\boldsymbol{b}}
\newcommand{\bc}{\boldsymbol{c}}
\newcommand{\bd}{\boldsymbol{d}}
\newcommand{\bes}{\boldsymbol{e}}     % special
\newcommand{\bef}{\boldsymbol{f}}     % special
\newcommand{\bg}{\boldsymbol{g}}
\newcommand{\bh}{\boldsymbol{h}}

\newcommand{\boldi}{\boldsymbol{i}}     % versori
\newcommand{\boldj}{\boldsymbol{j}}
\newcommand{\boldk}{\boldsymbol{k}}

\newcommand{\bl}{\boldsymbol{l}}
%\newcommand{\bm}{\boldsymbol{m}}      %
\newcommand{\bn}{\boldsymbol{n}}      % versore normale

\newcommand{\bp}{\boldsymbol{p}}
\newcommand{\bq}{\boldsymbol{q}}      % coord. di Lagrange
\newcommand{\br}{\boldsymbol{r}}
\newcommand{\bs}{\boldsymbol{s}}
\newcommand{\bt}{\boldsymbol{t}}
\newcommand{\bu}{\boldsymbol{u}}
\newcommand{\bv}{\boldsymbol{v}}
\newcommand{\bw}{\boldsymbol{w}}
\newcommand{\bx}{\boldsymbol{x}}     %%% Vettori
\newcommand{\by}{\boldsymbol{y}}
\newcommand{\bz}{\boldsymbol{z}}

% Uppercase letters
\newcommand{\bA}{\boldsymbol{A}}     %%% Matrici
\newcommand{\bB}{\boldsymbol{B}}
\newcommand{\bC}{\boldsymbol{C}}
\newcommand{\bD}{\boldsymbol{D}}
\newcommand{\bE}{\boldsymbol{E}}
\newcommand{\bF}{\boldsymbol{F}}      %
\newcommand{\bG}{\boldsymbol{G}}
\newcommand{\bH}{\boldsymbol{H}}
\newcommand{\bI}{\boldsymbol{I}}
\newcommand{\bJ}{\boldsymbol{J}}
\newcommand{\bK}{\boldsymbol{K}}
\newcommand{\bL}{\boldsymbol{L}}
\newcommand{\bM}{\boldsymbol{M}}
\newcommand{\bN}{\boldsymbol{N}}

\newcommand{\bP}{\boldsymbol{P}}
\newcommand{\bQ}{\boldsymbol{Q}}
\newcommand{\bR}{\boldsymbol{R}}
\newcommand{\bS}{\boldsymbol{S}}
\newcommand{\bT}{\boldsymbol{T}}
\newcommand{\bU}{\boldsymbol{U}}
\newcommand{\bV}{\boldsymbol{V}}      %  velocita'
\newcommand{\bW}{\boldsymbol{W}}
\newcommand{\bX}{\boldsymbol{X}}
\newcommand{\bY}{\boldsymbol{Y}}
\newcommand{\bZ}{\boldsymbol{Z}}

% Zero
\newcommand{\bzero}{\boldsymbol{0}}

\newcommand{\bvp}{\boldsymbol{\varpi}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Shorthands for bold letters with boldmath    %%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%% ********** WARNING  ************
%% Use either this file boldmath.tex or file mathbf.tex, BUT NOT BOTH!!!
%
%% Latin lowercase letters
%\newcommand{\ba}{\boldmath{a}}
%\newcommand{\bb}{\boldmath{b}}
%\newcommand{\bc}{\boldmath{c}}
%\newcommand{\bd}{\boldmath{d}}
%\newcommand{\bes}{\boldmath{e}}     % special
%\newcommand{\bef}{\boldmath{f}}     % special
%\newcommand{\bg}{\boldmath{g}}
%\newcommand{\bh}{\boldmath{h}}
%
%\newcommand{\bi}{\boldmath{i}}     % versori
%\newcommand{\bj}{\boldmath{j}}
%\newcommand{\bk}{\boldmath{k}}
%
%\newcommand{\bl}{\boldmath{l}}
%\newcommand{\bm}{\boldmath{m}}      %
%\newcommand{\bn}{\boldmath{n}}      % versore normale
%
%\newcommand{\bp}{\boldmath{p}}
%\newcommand{\bq}{\boldmath{q}}      % coord. di Lagrange
%\newcommand{\br}{\boldmath{r}}
%\newcommand{\bs}{\boldmath{s}}
%\newcommand{\bt}{\boldmath{t}}
%\newcommand{\bu}{\boldmath{u}}
%\newcommand{\bv}{\boldmath{v}}
%\newcommand{\bw}{\boldmath{w}}
%\newcommand{\bx}{\boldmath{x}}     %%% Vettori
%\newcommand{\by}{\boldmath{y}}
%\newcommand{\bz}{\boldmath{z}}
%
%% Uppercase letters
%\newcommand{\bA}{\boldmath{A}}     %%% Matrici
%\newcommand{\bB}{\boldmath{B}}
%\newcommand{\bC}{\boldmath{C}}
%\newcommand{\bD}{\boldmath{D}}
%\newcommand{\bE}{\boldmath{E}}
%\newcommand{\bF}{\boldmath{F}}      %
%\newcommand{\bG}{\boldmath{G}}
%\newcommand{\bH}{\boldmath{H}}
%\newcommand{\bI}{\boldmath{I}}
%\newcommand{\bJ}{\boldmath{J}}
%\newcommand{\bK}{\boldmath{K}}
%\newcommand{\bL}{\boldmath{L}}
%\newcommand{\bM}{\boldmath{M}}
%\newcommand{\bN}{\boldmath{N}}
%
%\newcommand{\bP}{\boldmath{P}}
%\newcommand{\bQ}{\boldmath{Q}}
%\newcommand{\bR}{\boldmath{R}}
%\newcommand{\bS}{\boldmath{S}}
%\newcommand{\bT}{\boldmath{T}}
%\newcommand{\bU}{\boldmath{U}}
%\newcommand{\bV}{\boldmath{V}}      %  velocita'
%\newcommand{\bW}{\boldmath{W}}
%\newcommand{\bX}{\boldmath{X}}
%\newcommand{\bY}{\boldmath{Y}}
%\newcommand{\bZ}{\boldmath{Z}}
%
%% Zero
%\newcommand{\bzero}{\boldmath{0}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Shorthands for dotted letters %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Dotted letters

\newcommand{\dbq}{\dot{\bq}}
\newcommand{\dbw}{\dot{\bw}}
\newcommand{\dbx}{\dot{\bx}}     %%% derivate temporali

\newcommand{\ddbq}{\ddot{\bq}}
\newcommand{\ddbw}{\ddot{\bw}}
%%\newcommand{\dbx}{\mathbf{\dot{x}}}  % NON sono uguali
\newcommand{\ddbx}{\ddot{\bx}}


\newcommand{\dep}{\dot{p}}
\newcommand{\dq}{\dot{q}}
\newcommand{\ded}{\dot{d}}
\newcommand{\dg}{\dot{g}}
\newcommand{\dr}{\dot{r}}
\newcommand{\ds}{\dot{s}}
\newcommand{\du}{\dot{u}}
\newcommand{\dv}{\dot{v}}
\newcommand{\dw}{\dot{w}}
\newcommand{\dx}{\dot{x}}
\newcommand{\dy}{\dot{y}}
\newcommand{\dz}{\dot{z}}

\newcommand{\dR}{\dot{R}}
\newcommand{\dX}{\dot{X}}

\newcommand{\ddx}{\ddot{x}}
\newcommand{\ddy}{\ddot{y}}
\newcommand{\ddz}{\ddot{z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Shorthands for hatted letters %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% lowercase letters
\newcommand{\hd}{\widehat{d}}
\newcommand{\hp}{\widehat{p}}

% capital letters
\newcommand{\hV}{\widehat{V}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Shorthands for bar letters %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% lowercase letters
\newcommand{\barp}{{\bar{p}}}
\newcommand{\barv}{{\bar{v}}}
\newcommand{\barn}{{\bar{n}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Shorthands for dotted bar letters %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\dbarp}{\dot{\barp}}
\newcommand{\dbarv}{\dot{\barv}}
\newcommand{\dbarn}{\dot{\barn}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Shorthands for check letters %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% lowercase letters
\newcommand{\chu}{{\check{u}}}
\newcommand{\chv}{{\check{v}}}
\newcommand{\chvphi}{{\check{\vphi}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Shorthands for tilde letters %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% lowercase letters
\newcommand{\tq}{{\bar{q}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Shorthands for sanserif letters %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% San serif lowercase letters
\newcommand{\sfa}{\mathsf{a}}
\newcommand{\sfb}{\mathsf{b}}
\newcommand{\sfc}{\mathsf{c}}
\newcommand{\sfd}{\mathsf{d}}
\newcommand{\sfe}{\mathsf{e}}
\newcommand{\sff}{\mathbf{f}}
\newcommand{\sfg}{\mathsf{g}}
\newcommand{\sfh}{\mathsf{h}}
\newcommand{\sfi}{\mathsf{i}}
\newcommand{\sfj}{\mathsf{j}}
\newcommand{\sfk}{\mathsf{k}}
\newcommand{\sfl}{\mathsf{l}}
\newcommand{\sfm}{\mathsf{m}}
\newcommand{\sfn}{\mathsf{n}}

\newcommand{\sfp}{\mathsf{p}}
\newcommand{\sfq}{\mathsf{q}}
\newcommand{\sfr}{\mathsf{r}}
\newcommand{\sfs}{\mathsf{s}}
\newcommand{\sft}{\mathsf{t}}
\newcommand{\sfu}{\mathsf{u}}
\newcommand{\sfv}{\mathsf{v}}
\newcommand{\sfw}{\mathsf{w}}
\newcommand{\sfx}{\mathsf{x}}
\newcommand{\sfy}{\mathsf{y}}
\newcommand{\sfz}{\mathsf{z}}

% Sans serif uppercase letters
\newcommand{\sfA}{\mathsf{A}}
\newcommand{\sfB}{\mathsf{B}}
\newcommand{\sfC}{\mathsf{C}}
\newcommand{\sfF}{\mathsf{F}}
\newcommand{\sfG}{\mathsf{G}}
\newcommand{\sfN}{\mathsf{N}}
\newcommand{\sfR}{\mathsf{R}}
\newcommand{\sfS}{\mathsf{S}}
\newcommand{\sfT}{\mathsf{T}}
\newcommand{\sfY}{\mathsf{Y}}
\newcommand{\sfZ}{\mathsf{Z}}

% Zero
\newcommand{\sfzero}{\mathsf{0}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Shorthands for outlined bold letters %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\bbR}{\mathbb{R}}    % Insieme dei numeri reali
\newcommand{\bbC}{\mathbb{C}}
\newcommand{\bbE}{\mathbb{E}}
\newcommand{\bbN}{\mathbb{N}}
\newcommand{\bbZ}{\mathbb{Z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Shorthands for calligraphic letters %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\calG}{\mathcal{G}}    % Insieme delle funzioni continue
\newcommand{\calL}{\mathcal{L}}    % Insieme delle funzioni integrabili in dominio illimitato
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calB}{\mathcal{B}}    % rigid body B
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Shorthands for fraktur letters %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\frakg}{\mathfrak{g}}    % Esempio di Lie algebra
\newcommand{\frakh}{\mathfrak{h}}    % Esempio di un'altra Lie algebra
\newcommand{\frakso}{\mathfrak{so}}  % Lie algebra di SO
\newcommand{\frakse}{\mathfrak{se}}  % Lie algebra di SE

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%% Shorthands for mathematical operators %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\DeclareMathOperator{\Ad}{Ad}
\DeclareMathOperator{\ad}{ad}
\DeclareMathOperator{\rank}{rank}

\renewcommand{\Re}{\operatorname{Re}}  % Parte reale, Reynolds
\renewcommand{\Im}{\operatorname{Im}}  % Parte immaginaria
\newcommand{\Ma}{\operatorname{Ma}}    % Mach

\newcommand{\tr}{\operatorname{tr}}  %% traccia

\newcommand{\dd}{\text{{\sl d}}}        %% differenziale

\newcommand{\grad}{\operatorname{grad}} %% gradiente
\newcommand{\rot}{\operatorname{rot}}   %% rotore
\renewcommand{\div}{\operatorname{div}} %% divergenza

\newcommand{\inv}{\operatorname{inv}}   %% involute
\newcommand{\Cos}{\operatorname{c}}      %% abbreviazione Cos
\newcommand{\Sin}{\operatorname{s}}      %% abbreviazione Sin
\newcommand{\vect}{\operatorname{vect}}

\newcommand{\ST}{\scriptstyle}
\newcommand{\D}{\displaystyle}

\newcommand{\ti}{\tilde}      % accento matematico in breve

\def\pd{\partial}
\def\at{\bigg|}      % serve per dire dove va valutata una derivata.

\newcommand{\rT}{\text{T}}   % T di trasposta

\newcommand{\nnum}{\nonumber \\}
\newcommand{\Nnum}[1]{\nonumber \\[#1]}

\newcommand{\ov}[1]{\overline{#1}}

\providecommand{\norm}[1]{\lVert#1\rVert}  % definisce i delimitatori di una norma

\newcommand{\p}{^{\!\cdot\!}}  % punto STRETTO in alto nei numeri lunghi: 1\p000
\newcommand{\pp}{^{\mspace{-1.0mu}\cdot\mspace{-1.0mu}}}
%\makeatletter
%\newcommand{\pp}{^{@!\cdot@!}}  % punto in alto nei numeri lunghi: 2\pp000
%\makeatother

